HadamRNN: Binary and Sparse Ternary Orthogonal RNNs

Binary and sparse ternary weights in neural networks enable faster computations and lighter representations, facilitating their use on edge devices with limited computational power. Meanwhile, vanilla RNNs are highly sensitive to changes in their recurrent weights, making the binarization and ternarization of these weights inherently challenging. To date, no method has successfully achieved binarization or ternarization of vanilla RNN weights. We present a new approach leveraging the properties of Hadamard matrices to parameterize a subset of binary and sparse ternary orthogonal matrices. This method enables the training of orthogonal RNNs (ORNNs) with binary and sparse ternary recurrent weights, effectively creating a specific class of binary and sparse ternary vanilla RNNs. The resulting ORNNs, called HadamRNN and Block-HadamRNN, are evaluated on benchmarks such as the copy task, permuted and sequential MNIST tasks, the IMDB dataset, two GLUE benchmarks, and two IoT benchmarks. Despite binarization or sparse ternarization, these RNNs maintain performance levels comparable to state-of-the-art full-precision models, highlighting the effectiveness of our approach. Notably, our approach is the first solution with binary recurrent weights capable of tackling the copy task over 1000 timesteps.

==> main_content/background.tex <==
\section{The difficulty of designing binary ORNNs}

Orthogonal recurrent networks are a class of recurrent networks, that rely on the same recurrent operation as the one of a vanilla recurrent network, but add an orthogonality constraint on the recurrent weight matrix. Given a sequence of inputs $x_t, \ldots, x_T \in \RR^{d_{in}}$, the model computes a sequence of hidden states $h_1, \ldots, h_T \in \RR^{d_h}$ according to
\begin{equation*}
    \label{eq:ORNN_hidden}
    h_{t}  = \sigma \left( W h_{t-1} + U x_{t} + b \right),
\end{equation*}
where the recurrent weight matrix $W$ is constrained to be orthogonal.

Thanks to the orthogonality of the recurrent weight matrix, these networks were shown to be able to solve complex very long-term dependency tasks such as the copy task with $1000$ timesteps and more \cite{lezcano2019cheap, helfrich2018orthogonal, Vorontsov2017OnOA, DBLP:conf/icml/MhammediHRB17}, in addition to have a very simple formulation with inference complexity linear in the length of the sequence. Besides, binarization, that is, representing weights with a single bit, represents the most extreme form of quantization and, as a result, offers the highest degree of compression achievable through quantization. This makes the binarization of ORNNs compelling.

However, \cite{foucault2024quantized} suggested that ORNN quantization is a difficult problem, as applying classic quantization schemes to orthogonal matrices generally result in matrices that are not orthogonal. The authors empirically demonstrate that as the bitwidth of quantization decreases, matrices deviate further from orthogonality, thereby undermining the benefits associated with maintaining orthogonality. For this reason, the experimental findings in \cite{foucault2024quantized} reveal a sharp decline in performance as the bitwidth is reduced.

As a result, a binarization scheme such as the one in \cite{rastegari2016xnor} can not be applied in a straightforward manner to the recurrent weight matrix of an ORNN, as this would result in a matrix far from orthogonal, and hence the network would suffer from the traditional issues in vanilla recurrent networks such as the Vanishing / Exploding gradient problems.

Instead of quantizing full-precision weights at inference time, we propose another approach to optimize the binary recurrent weight matrix. We initialize the matrix as a \textbf{Hadamard matrix} (binary and orthogonal) and we apply elementary trainable linear transformations to this matrix that preserve both orthogonality and binarity throughout learning. In this manner we are able to optimize the model over the set of Hadamard matrices.

==> main_content/background_old.tex <==
\section{Background}
\label{sec:background}


\red{Réecrire toute cette section en 2 sous sections (la renommer éventuellement en preliminaries, un peu comme dans QORNNs): \\1/ ORNNs \\  2/ quantification \\ En particulier, pas besoin de décrire les vanilla RNNs et le vanishing / exploding gradient problem dans le corps de l'article, il faut en venir directement au fait}

We briefly describe the fundamental mechanisms of a two layers vanilla RNN, the vanishing / exploding gradient problems and how orthogonality of the recurrent weight matrix help mitigate these issues.


\subsection{$2$-layers Vanilla RNNs}

A $2$-layers vanilla RNN is a function that takes as input a sequence of $T$ $d_{in}-$dimensional points $(x_1, \ldots, x_T)~\in~(\RR^{d_{in}})^{T}$, and outputs either a sequence $(y_1, \ldots, y_T)~\in~(\RR^{d_o})^T$ or a single point $y_T \in \RR^{d_o}$.

A $2$-layers vanilla RNN is defined by a neural network architecture relying on a set of parameters including an input-to-hidden matrix $U \in \RR^{d_h \times d_{in}}$ ($d_h$ is the hidden layer dimension, or hidden size for brevity), a recurrent weight matrix $W \in \RR^{d_h \times d_h}$, a hidden-to-output matrix $V \in \RR^{d_o \times d_h}$, an inner bias $b \in \RR^{d_h}$, an outer bias $b_o \in \RR^{d_o}$, and an activation function $\sigma : \RR^{d_h} \rightarrow \RR^{d_h}$. A vanilla RNN computes a sequence of hidden states $(h_1, \ldots, h_T)$ according to
\begin{equation}
    \label{eq:vanilla_rnn}
    h_t = \sigma \left( W h_{t-1} + U x_t + b \right) \in \RR^{d_h},
\end{equation}
for each timestep $t = 1, \ldots, T$ and $h_0$ initialized as the zero vector. In each of our experiments, $\sigma$ is the $ReLU$ activation function.

The output $y_t$ is computed using
\begin{equation}
    \label{eq:rnn_output}
    y_t = \sigma_o \left( V h_t + b_o \right) \in \RR^{d_o},
\end{equation}
for each timestep $t=1, \ldots, T$ in \textit{many-to-many} tasks (a prediction is made for each timestep), and for $t=T$ in \textit{many-to-one} tasks (only one prediction is associated to the input sequence). $\sigma_o$ is the identity function for regression tasks, and it is the softmax activation function for classification tasks.

\subsection{The Vanishing / Exploding gradient problems and orthogonal RNNs}
Training vanilla recurrent neural networks is notoriously difficult due to the vanishing and the exploding gradient problems \cite{pascanu2013difficulty}. We briefly summarize how these issues arise and why orthogonality allows to circumvent them. Training a vanilla RNN involves minimizing an objective function $C$ with respect to the network's parameters. This involves the computation of the gradient $\frac{\partial C}{\partial h_t}$ for all $t = 1, \ldots, T$. One can show \cite{arjovsky2016unitary} that
\begin{equation}
    \label{eq:rnn_gradient}
    \frac{\partial C}{\partial h_t} = \frac{\partial C}{\partial h_T} \prod_{k=t}^{T-1} D_{k} W^\top,
\end{equation}
where $D_k = diag \left( \sigma'\left( W h_{k} + U x_{k+1} + b \right) \right)$ is the Jacobian matrix of the activation $\sigma$ between timesteps $k$ and $k+1$. This means that if $D_k$ has diagonal values that are close to $1$ for all $k=t, \ldots, T$, then the contribution of the $D_k$'s in the corresponding directions are negligible \textcolor{red}{Discuter de cette hypothèse en appendix ?}. $\frac{\partial C}{\partial h_t}$ thus depends almost exponentially on $W$ in these directions, which may cause severe numerical instability as soon as $W$ has eigenvalues that are either significantly higher than $1$, or significantly smaller than $1$ \cite{helfrich2018orthogonal}. A simple way to work around this issue is to constrain $W$ to be orthogonal, namely, to impose $W W^\top = I$, where $I$ denotes the identity matrix. In that case, $W$ has the desirable property that all its eigenvalues have absolute value equal to $1$, which efficiently limitate the above-mentioned vanishing and exploding gradient problems.

A range of studies have proposed a variety of methods to construct ORNNs, that is, vanilla RNNs with orthogonal recurrent weight matrix $W$. These typically include parametrization of the orthogonal group or a subset of it \cite{DBLP:conf/icml/MhammediHRB17, helfrich2018orthogonal, lezcano2019cheap}, or projection of $W$ onto the orthogonal group \cite{kiani2022projunn, foucault2024quantized}. These studies contribute to a broader line of research  focusing on imposing the recurrent weight matrix to be unitary \cite{arjovsky2016unitary, wisdom2016fullcapacity, jing2017tunable}, encompassing complex-valued matrices with eigenvalues having modulus $1$. We now explain how we construct our HadamRNNs, that is, orthogonal RNNs with binary recurrent weight matrix.





%\red{Vanishing / Exploding gradients - alternative paragraph:}

%where $D_k = diag \left( \sigma'\left( W h_{k} + U x_{k+1} + b \right) \right)$ is the (diagonal) Jacobian matrix of the activation $\sigma$ between timesteps $k$ and $k+1$. We let $\|.\|$ denote both the spectral radius norm for a matrix and the $L_2$ norm for a vector. Using the standard inequality $\|AB\| \leq \|A\| \|B\|$ for any two matrices $A, B$, \cite{arjovsky2016unitary} show that
%\begin{align*}
 %   \label{eq:gradient_up_bound}
  %  \left\|\frac{\partial C}{\partial h_t}\right\| \leq \lambda^{T-t} \left\| \frac{\partial C}{\partial h_T}\right\| \prod_{k=t}^{T-1} \left\| D_k \right\|,
%\end{align*}
%where $\lambda$ is the highest singular value of $W$. If


==> main_content/experiments_old.tex <==
\section{Experiments}
\label{sec:expe}


In this section, we evaluate the performance of our HadamRNN on four benchmarks of different kinds. Three of these require retaining information for extended delays, while one is a language modeling problem that can be learnt with a short-term memory model. We conduct experiments on three classification tasks and one regression task.

\red{To serve as a baseline, we also present the results of a full-precision LSTM, and those of a full-precision ORNN trained with the ProjUNN-D algorithm, as introduced in \cite{kiani2022projunn}.}

All our models were trained using the Adam optimizer \cite{2014arXiv1412.6980K}. Hyperparameters selection was made using validation sets on each tasks.
More details on the hyperparameters and implementations can be found in \cref{app:expe_details}.


\subsection{Copy task}
\label{seq:copy_task}

The Copy task is a standard sequential problem that was first introduced in \cite{hochreiter1997long}. This task requires to memorize information over long large numbers of timesteps, and vanilla LSTMs notoriously struggle to solve it \cite{arjovsky2016unitary, helfrich2018orthogonal, lezcano2019cheap}. We follow the setup of \cite{lezcano2019cheap}, in which the data sequences are constructed as follows. We consider an alphabet $\left\{a_k\right\}_{k=0}^9$ of $10$ characters. Given a sentence lenght $K$ and a delay $L$, an input sequence has its first $K$ elements sampled uniformly and independently from $\left\{a_k\right\}_{k=1}^8$, followed by $L$ repetitions of the \textit{blank} character $a_0$, $1$ repetition of the \textit{marker} character $a_9$ and finally $K-1$ repetitions of $a_0$. The first $K$ elements is a sentence that the network has to memorize and reproduce identically after outputting $L + K$ instances of $a_0$. In other words, the model processes the elements one at a time and has to output $a_0$ at each timestep until it gets $a_9$ as input. Then the model is required to start outputting the input sentence (the ten first elements of the input sequence). An example of possible input / output sequences for $K = 4$, $L = 6$ and an alphabet $\{-ABCDEFGH:\}$ is given below:
\begin{align*}
    \label{ex:copy_task}
    \text{input: } ACFB------:--- \\
    \text{output: } ----------ACFB
\end{align*}

We use the average cross entropy to measure the error between an input sequence and its associated prediction. A naive strategy would be to predict $L+K$ occurrences $a_0$ followed by $K$ randomly selected items from $\left\{a_k\right\}_{k=1}^8$, which yields an expected cross entropy of $\frac{K \log 8}{L + 2K}$. We use this score as a naive baseline to assess if the task is learnt.

In our experiments, we fixed $K=10$ and $L+2K=1000$. We used a hidden size $n_h = 512$. \red{autres elmts d'implém et commenter résultats} Results are summarized in \cref{tab:copy_task_performance}.


\begin{table}
  \caption{Performances of HadamRNN with hidden size $n_h = 512$ and benchmark models on the Copy task with $T=1000$ timesteps. Models are assessed using the cross entropy.}
    \label{tab:copy_task_performance}
  \centering
  
  \begin{tabular}{l c c c c c}  
    \toprule

    Dataset & & & & \textbf{Copy task ($T= 1000$)} &  \\
    \midrule
    \midrule
    Model & $\#$ PARAMS &  size (Kbytes) & & \\
    \midrule
    \midrule
    naive baseline & - & - & & $2.08e-2$ \\
 \midrule
 \multirow{1}{*}{LSTM \red{source ?}} & & & & \\
 \multirow{1}{*}{EXPRNN \cite{lezcano2019cheap}} & & & & \\
 \multirow{1}{*}{ProjUNN \cite{kiani2022projunn}} & & & & \\
 \multirow{1}{*}{HadamRNN (ours)} & & & & \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Adding task}

The Adding task, introduced in \cite{hochreiter1997long}, is a regression task based on a synthetic dataset. We follow the setup of \cite{arjovsky2016unitary} in which sequences are constructed as follows. An input sequence of length $T$ $\left(x_t\right)_{t=1}^T \in (\RR^2)^T$ is the stack of two $1$-dimensional data sequences $(x_1[1], \ldots, x_T[1])$ and $(x_1[2], \ldots, x_T[2])$ respectively. The first sequence $\left(x_t[1]\right)_{t=1}^T$ consists of random numbers sampled uniformly and independently from the interval $[0,1]$. The second sequence $\left(x_t[2]\right)_{t=1}^T$ contains only $0$ entries except for two, selected at random respectively in the first and the second half of the sequence, which are set to $1$. Given such a sequence, the task is to output the sum of the two scalars of the first sequence which are located at the same inidices as the $1$ from the second sequence, that is, $\sum_{t=1}^T x_t[1] \cdot x_t[2]$. Naively predicting $1$ regardless of the input sequence yields an expected mean squared error (MSE) of $0.167$, this serves as a baseline to assess if the task is learnt.

Following common practice \cite{helfrich2018orthogonal, kiani2022projunn}, we set $T = 750$ in all our experiments. We used a hidden size $n_h = 256$.
\red{autres elmts d'implém et commenter les résultats}
Results are summarized in \cref{tab:adding_task_performance}.

\begin{table}
  \caption{Performances of HadamRNN with hidden size $n_h = 256$ and benchmark models on the Adding task with $T=750$ timesteps. Models are assessed using the mean squared error.}
    \label{tab:adding_task_performance}
  \centering
  
  \begin{tabular}{l c c c c c}  
    \toprule

    Dataset & & & & \textbf{Adding task ($T= 750$)} &  \\
    \midrule
    \midrule
    Model & $\#$ PARAMS &  size (Kbytes) & & \\
    \midrule
    \midrule
    naive baseline & - & - & & $0.167$ \\
 \midrule
 \multirow{1}{*}{LSTM \red{source ?}} & & & & \\
 \multirow{1}{*}{ProjUNN \cite{kiani2022projunn}} & & & & \\
 \multirow{1}{*}{HadamRNN (ours)} & & & & \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Permuted sequential MNIST (pMNIST)}

The permuted sequential MNIST task is another classic long-term memory task. The dataset here is the MNIST dataset in which the $28 \times 28$ images are flattenend into $784$-long sequences of $1$-dimensional pixels (scalars normalized in $[0,1]$). The pixels within a sequence are then randomly shuffled according to a fixed permutation; we use the same one as in \cite{kiani2022projunn}. As in the vanilla MNIST task, the goal here is for the model to output the correct hand-written digit within the image. The prediction error is measured using the cross entropy, and the model's performance is evaluated with the accuracy.

We used a hidden size $n_h = 512$. \red{Details d'implém}
Results are summarized in \cref{tab:pmnist_performance}.

\begin{table}
  \caption{Performances of HadamRNN with hidden size $n_h = 512$ and benchmark models on the Permuted (sequential) MNIST task. Models are assessed using the cross entropy.}
    \label{tab:pmnist_performance}
  \centering
  
  \begin{tabular}{l c c c c c}  
    \toprule

    Dataset & & & & \textbf{permuted MNIST} &  \\
    \midrule
    \midrule
    Model & $\#$ PARAMS &  size (Kbytes) & & \\
    \midrule
    \midrule
 \multirow{1}{*}{LSTM \red{source ?}} & & & & \\
 \multirow{1}{*}{EXPRNN \cite{lezcano2019cheap}} & & & & \\
 \multirow{1}{*}{ProjUNN \cite{kiani2022projunn}} & & & & \\
 \multirow{1}{*}{HadamRNN (ours)} & & & & \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Character level Penn TreeBank}

Finally, we benchmark our HadamRNN on a language modeling task. The Penn TreeBank corpus \cite{Taylor2003ThePT} is a text dataset composed of sentences, using $50$ different characters. Each sentence is processed as a sequence in which the elements are the characters, one-hot-encoded as $50$-dimensional vectors. The goal is to predict the next characters given the previous ones. Following common practice \cite{Ott2016RecurrentNN, ardakani2018learning}, we split the dataset into $5017$k, $393$k and $442$k training, validation and test characters respectively. The sentences are splitted into sequences of $50$ characters each; shorter senquences are extended using padding with a dummy character. We use the cross entropy to learn the task, and we use the Bit-per-character (BPC) metric to evaluate our model.

We used a hidden size $n_h = 1024$.
\red{Details d'implém}
Results are summarized in \cref{tab:ptb_performance}.

\begin{table}
  \caption{Performances of HadamRNN with hidden size $n_h = 1024$ and benchmark models on the Character level Penn TreeBank. Models are assessed using the Bit Per Character (BPC) metric.}
    \label{tab:ptb_performance}
  \centering
  
  \begin{tabular}{l c c c c c}  
    \toprule

    Dataset & & & & \textbf{Adding task ($T= 750$)} &  \\
    \midrule
    \midrule
    Model & $\#$ PARAMS &  size (Kbytes) & & \\
    \midrule
    \midrule
    \multirow{1}{*}{LSTM \red{source ?}} & & & & \\
 \multirow{1}{*}{1vfRNN \cite{10.5555/3122009.3242044}} & & & & \\
 \multirow{1}{*}{HadamRNN (ours)} & & & & \\
    \bottomrule
  \end{tabular}
\end{table}
